COAST: Constraints and Streams for Task and Motion Planning

Task and Motion Planning (TAMP) algorithms solve long-horizon robotics tasks by integrating task planning with motion planning; the task planner proposes a sequence of actions towards a goal state and the motion planner verifies whether this action sequence is geometrically feasible for the robot. However, state-of-the-art TAMP algorithms do not scale well with the difficulty of the task and require an impractical amount of time to solve relatively small problems. We propose Constraints and Streams for Task and Motion Planning (COAST), a probabilistically-complete, sampling-based TAMP algorithm that combines stream-based motion planning with an efficient, constrained task planning strategy. We validate COAST on three challenging TAMP domains and demonstrate that our method outperforms baselines in terms of cumulative task planning time by an order of magnitude. You can find more supplementary materials on our project \href{https://branvu.github.io/coast.github.io}{website}.

==> figures/5-plan.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/SuccessPlans_New.pdf}
        \caption{
            Number of iterations to solve each domain (\textit{Block}, \textit{Kitchen}, \textit{Rover}) are presented. On the x-axis we increase the difficulty, and on the y-axis we measure the median number of iterations the planner took to find a solution with a 50\% confidence interval. Our method uses the least number of iterations to solve the same problems compared to PDDLStream and IDTMP. For the \textit{Block} domain with 5 obstacles, IDTMP requires 200 iterations and PDDLStream requires 50 iterations, whereas our method only requires 10 iterations.   
        }
    \label{fig:plans}
\end{figure}

==> tex/5-domains.tex <==
We evaluate our algorithm on three domains (\textit{Blocks}, \textit{Kitchen}, \textit{Rover}) that test a range of difficulty, including large tasks spaces (\textit{Kitchen}, \textit{Rover}), non-monotonicity (\textit{Block}, \textit{Kitchen}), task-motion complexity (\textit{Block}, \textit{Rover}), infeasible actions (\textit{Block}, \textit{Rover}), and non-geometric actions (\textit{Kitchen}). We refer readers to the TAMP Benchmark~\cite{benchmark} for in-depth explanations of these criteria and the supplementary material on the webpage for examples of the domains.  
%We focus on several important factors of TAMP problems for our domains that are suggested by standard TAMP benchmarks \cite{benchmark}. These factors include large task spaces, non-monotonicity, task-motion complexity, infeasible actions, and non-geometric actions. Large task spaces simulate real world settings where robots can interact with many objects in the scene. Non-monotonicity refers to tasks where an object has to change locations throughout the plan. This is important because this means that we cannot make an assumption that once an object is moved, it will not need to be considered anymore. Task-motion complexity refers to the amount of dependencies between symbolic actions and geometric feasibility. An example of high task-motion complexity are domains that have obstructions. Infeasible actions occur where there are geometric constraints that prevent a symbolic action from being applied. Lastly, non-geometric actions are actions that are purely symbolic. These are still important to consider because non-geometric actions can update the symbolic state and send key information to the user. An example of this is checking for failure states in industrial applications. 


% \subsection{Sort Clutter}
% This domain is proposed by the TAMP Benchmark~\cite{benchmark}. The scene contains four tables (\pddl{left}, \pddl{right}, \pddl{front}, \pddl{back}) with $N$ blue blocks, $N$ green blocks, and $2N$ red blocks. All of the blocks are given random locations on the \pddl{front} or \pddl{back} tables. The goal is to move the blue blocks to the \pddl{left} and the \pddl{green} blocks to the \pddl{right} table while avoiding collisions with the red blocks. Because there are so many objects, this domain has a large task space. The robot is also mounted on a mobile base, which adds to the task-motion complexity.
%is difficult because it has a large task space with many blocks to pick and many potential poses to place. This domain features a robot arm with a mobile base, which makes collision avoidance and planning challenging.
